A Fully Anisotropic Formulation of Stochastic Cell Rescaling

Anisotropic barostats are employed to carry out Molecular Dynamics simulations where the volume is allowed to fluctuate with no constraints on the shape of the simulation cell. Most of these algorithms are based on second-order differential equations and share some common drawbacks, namely they can lead to slowly damped oscillations in the equilibration phase, and they do not allow to control efficiently the volume autocorrelation time. This work develops the anisotropic version of stochastic cell rescaling, a first-order stochastic barostat that overcomes these limits and can also be employed in the production phase, resulting in the correct physical fluctuations of the cell. The algorithm can be easily implemented in the existing codes on top of the anisotropic Berendsen barostat. The validation tests, performed on a number of crystal systems, show that the method is robust against wide variations of the input parameter, which allows an efficient control of the volume autocorrelation time.

==> conclusions/conclusions.tex <==
% This is where you conclude your thesis.



==> core/declaration_of_authorship/declaration_of_authorship.tex <==
I hereby declare that this thesis is my own unaided work. All direct or indirect sources used are acknowledged as references.\\[6 ex]

\begin{flushleft}
    Potsdam, \today
    \hspace*{2 em}
    \raisebox{-0.9\baselineskip}
    {
        \begin{tabular}{p{5 cm}}
            \hline
            \centering\footnotesize\printAuthor
        \end{tabular}
    }
\end{flushleft}

==> introduction/introduction.tex <==
% Here you introduce your topic to the reader.



==> preface/abstract.tex <==
% This file should contain the English abstract.



==> preface/abstractGerman.tex <==
% This file should contain the German abstract.


